Complexity of Classical Acceleration for $\ell_1$-Regularized PageRank

We study the degree-weighted work required to compute $\ell_1$-regularized PageRank using the standard accelerated proximal-gradient method (FISTA). For non-accelerated methods (ISTA), the best known worst-case work is $\widetilde{O}((\alpha\rho)^{-1})$, where $\alpha$ is the teleportation parameter and $\rho$ is the $\ell_1$-regularization parameter. It is not known whether classical acceleration methods can improve $1/\alpha$ to $1/\sqrt{\alpha}$ while preserving the $1/\rho$ locality scaling, or whether they can be asymptotically worse. For FISTA, we show a negative result by constructing a family of instances for which standard FISTA is asymptotically worse than ISTA. On the positive side, we analyze FISTA on a slightly over-regularized objective and show that, under a confinement condition, all spurious activations remain inside a boundary set $\mathcal{B}$. This yields a bound consisting of an accelerated $(\rho\sqrt{\alpha})^{-1}\log(\alpha/\varepsilon)$ term plus a boundary overhead $\sqrt{vol(\mathcal{B})}/(\rho\alpha^{3/2})$. We also provide graph-structural sufficient conditions that imply such confinement.

==> definitions.tex <==
%
\usepackage{xparse}
\usepackage{xargs}

\makeatletter %
\def\Hy@raisedlink@left#1{%
    \ifvmode
        #1%
    \else
        \Hy@SaveSpaceFactor
        \llap{\smash{%
        \begingroup
            \let\HyperRaiseLinkLength\@tempdima
            \setlength\HyperRaiseLinkLength\HyperRaiseLinkDefault
            \HyperRaiseLinkHook
        \expandafter\endgroup
        \expandafter\raise\the\HyperRaiseLinkLength\hbox{%
            \Hy@RestoreSpaceFactor
            #1%
            \Hy@SaveSpaceFactor
        }%
        }}%
        \Hy@RestoreSpaceFactor
        \penalty\@M\hskip\z@ 
    \fi
}
\makeatother

\newcommand\newlink[2]{{\protect\hyperlink{#1}{\normalcolor #2}}}
\makeatletter
\newcommand\newtarget[2]{\Hy@raisedlink@left{\hypertarget{#1}{}}#2} %
%
\makeatother

%
%

\newcommand\linktoproof[1]{{\normalfont[{\hyperlink{proof:#1}{$\downarrow$}}]}}
\newcommand\linkofproof[1]{\textbf{of \cref{#1}. }\newtarget{proof:#1}}

%
\usepackage[bb=boondox]{mathalpha} %
%
\newcommand{\zeros}{\mathbb{0}} 

\newcommand{\bigo}[1]{{O}( #1 )}
\newcommand{\bigol}[1]{O\left( #1 \right)}
\newcommand{\bigop}[2]{\newlink{def:big_o_p}{O}_{#1}( #2 )}
\newcommand{\bigolp}[2]{\newlink{def:big_o_p}{O}_{#1}\left( #2 \right)}
\newcommand{\bigoast}[1]{\newlink{def:big_o_ast}{O^\ast}( #1 )}
\newcommand{\bigoastl}[1]{\newlink{def:big_o_ast}{O^\ast}\left( #1 \right)}
\newcommand{\bigotilde}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}( #1 )}
\newcommand{\bigotildel}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}\left( #1 \right)}
\newcommand{\bigotildelp}[2]{\newlink{def:big_o_tilde}{\widetilde{O}}_{#1}\left( #2 \right)}
\newcommand{\bigomegatilde}[1]{\newlink{def:big_o_tilde}{\widetilde{\Omega}}( #1 )}

\newcommand{\innp}[1]{\langle #1 \rangle}
\providecommand{\set}[1]{\{ #1 \}}
\newcommand\setl[1]{\left\{ #1 \right\}}
\newcommand\setsuch[2]{\{ #1 \mid #2  \}}
\newcommand\setsuchl[2]{\left\{ #1 \mid #2  \right\}}

%

\let\oldepsilon\epsilon
\renewcommand{\epsilon}{\newlink{def:accuracy_epsilon}{\oldepsilon}}

%
\newcommand{\Lips}{\newlink{def:Lipschitz_constant}{L_{\mathtt{p}}}} 

\let\strikedL\L
\renewcommand{\L}{\newlink{def:riemannian_smoothness_of_F}{L}} 


\newcommand{\astfenchel}{\newlink{def:asterisk_of_fenchel_dual}{\ast}}
\let\oldPi\Pi
\renewcommand{\Pi}{\newlink{def:euclidean_projection}{\oldPi}}
\newcommandx\Rp[1][1=, usedefault]{\R_{\geq 0}^{#1}}


\newcommand\indicator[1]{\newlink{def:indicator_function}{\operatorname{I}_{#1}}}
\newcommand\xast{\newlink{def:xast}{x^\ast}}
\newcommand\X{\mathcal{X}}
\newcommand*\dom{\operatorname{dom}}


%

\newcommand{\ip}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\prox}{\operatorname{prox}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\vol}{\operatorname{vol}}
\newcommand{\sign}{\operatorname{sign}}

\newcommand{\Istar}{I^\star}
\newcommand{\xstar}{x^\star}
\newcommand{\Sstar}{S^\star}


\newcommand\lapl{\newlink{def:laplacian_matrix}{\mathcal{L}}}

\newcommandx*\x[2][1=k, 2= , usedefault]{x^{( #1 )}_{#2}}
\newcommandx*\y[2][1=k, 2= , usedefault]{y^{( #1 )}_{#2}}
\newcommandx*\z[2][1=k, 2= , usedefault]{z^{( #1 )}_{#2}}

\newcommand{\N}{\mathcal{N}} %
\newcommand{\bdry}{\partial} %

\usepackage{silence}
\WarningFilter{latex}{Command \showhyphens has changed}

